Labelled Sequents for Inquisitive First-Order Modal Logic

In recent work, an inquisitive first-order modal logic has been proposed to reason about relations of modal dependence, including the notion of global supervenience (functional dependence among the extensions of predicates relative to a space of possibilities). At present, no proof system exists for this logic. We provide a complete labelled sequent calculus, extending a calculus developed by Litak and Sano for a weak version of inquisitive first-order logic. We prove strong completeness for the calculus and show that it enjoys desirable structural properties, including the invertibility of its rules and the admissibility of cut.

==> eptcsdata.tex <==
\providecommand{\firstpage}{242}
\providecommand{\publicationstatus}{M.~B\'ilkov\'a, M.~Gattinger, I.~van~der~Giessen, M.~Girlando, Y.~Wang (Eds.):\\
Advances in Modal Logic 2026 (AiML 2026)\\
EPTCS 447, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.447.14}{10.4204/EPTCS.447.14}}

